MasterKey: Automated Jailbreak Across Multiple Large Language Model Chatbots

Large Language Models (LLMs) have revolutionized Artificial Intelligence (AI) services due to their exceptional proficiency in understanding and generating human-like text. LLM chatbots, in particular, have seen widespread adoption, transforming human-machine interactions. However, these LLM chatbots are susceptible to "jailbreak" attacks, where malicious users manipulate prompts to elicit inappropriate or sensitive responses, contravening service policies. Despite existing attempts to mitigate such threats, our research reveals a substantial gap in our understanding of these vulnerabilities, largely due to the undisclosed defensive measures implemented by LLM service providers. In this paper, we present Jailbreaker, a comprehensive framework that offers an in-depth understanding of jailbreak attacks and countermeasures. Our work makes a dual contribution. First, we propose an innovative methodology inspired by time-based SQL injection techniques to reverse-engineer the defensive strategies of prominent LLM chatbots, such as ChatGPT, Bard, and Bing Chat. This time-sensitive approach uncovers intricate details about these services' defenses, facilitating a proof-of-concept attack that successfully bypasses their mechanisms. Second, we introduce an automatic generation method for jailbreak prompts. Leveraging a fine-tuned LLM, we validate the potential of automated jailbreak generation across various commercial LLM chatbots. Our method achieves a promising average success rate of 21.58%, significantly outperforming the effectiveness of existing techniques. We have responsibly disclosed our findings to the concerned service providers, underscoring the urgent need for more robust defenses. Jailbreaker thus marks a significant step towards understanding and mitigating jailbreak threats in the realm of LLM chatbots.

==> Tex/3-Empirical_Study.tex <==

\begin{table*}[t]
\caption{Usage policies of service providers}
\label{tab:policy}
\begin{adjustbox}{width=\linewidth}
\begin{threeparttable}
\begin{tabular}{l||cccccccc}
\toprule
\multirow{2}{*}{\textbf{Prohibited Scenarios}}                                                     & \multicolumn{2}{c}{\textbf{OpenAI}} & \multicolumn{2}{c}{\textbf{Google Bard}} & \multicolumn{2}{c}{\textbf{Bing Chat}} & \multicolumn{2}{c}{\textbf{Ernie}} \\
& Specified & Enforced & Specified & Enforced & Specified & Enforced & Specified & Enforced \\ \midrule

\textbf{Illegal} usage against Law                                            & \ding{51} & \ding{51}           & \ding{51} &  \ding{51}          & \ding{51} &     \ding{51}            & \ding{51} &  \ding{51}          \\
Generation of \textbf{Harmful} or Abusive Content                                        & \ding{51} & \ding{51}           & \ding{51} &  \ding{51}          & \ding{51} &     \ding{51}            & \ding{51} &  \ding{51}          \\
Generation of \textbf{Adult} Content                   & \ding{51} & \ding{51}           & \ding{51} &  \ding{51}          & \ding{51} &     \ding{51}            & \ding{51} &  \ding{51}          \\
Violation of Rights and \textbf{Privacy}                                       & \ding{51} & \ding{51}           & \ding{51} &  \ding{51}          & \ding{51} &     \ding{51}            & \ding{51} &  \ding{51}          \\
\textbf{Political} Campaigning/Lobbying                          & \ding{51} &   \ding{55}            & \ding{55} &  \ding{55}          & \ding{55} &    \ding{55}        & \ding{55} &    \ding{51}        \\
\textbf{Unauthorized Practice} of Law, Medical and Financial Advice & \ding{51} &   \ding{51}          & \ding{55} &  \ding{55}         & \ding{55} &   \ding{55}        & \ding{55} &   \ding{55}        \\
Restrictions on High Risk \textbf{government} Decision-making                    & \ding{51} &  \ding{55}         & \ding{55} &  \ding{55}         & \ding{55} &    \ding{55}       & \ding{51} &   \ding{51}        \\
Generation and Distribution of \textbf{Misleading} Content                 & \ding{55} &  \ding{55}        & \ding{51} &   \ding{55}        & \ding{51} &   \ding{55}        & \ding{51} &   \ding{51}        \\
Creation of \textbf{Inappropriate} Content                         & \ding{55} &   \ding{55}           & \ding{51} &  \ding{51}          & \ding{51} &   \ding{55}         & \ding{51} &  \ding{51}          \\
Content Harmful to \textbf{National Security} and Unity                                  & \ding{55} &  \ding{55}           & \ding{55} &  \ding{55}         & \ding{55} &   \ding{55}        & \ding{51} &  \ding{51}         \\  \bottomrule
\end{tabular}
  \end{threeparttable}
\end{adjustbox}
\end{table*}


\section{An Empirical Study}\label{sec:study}

%\lyk{need to unify/standardize the use of the following terms: LLM, LLM chatbot, LLM chatbot service}

To better understand the potential threats posed by jailbreak attacks as well as existing jailbreak defenses, we conduct a comprehensive empirical study. Our study centers on two critical research questions (RQ):

\begin{itemize}[leftmargin=*]
\item\textbf{RQ1 (Scope)} What are the usage policies set forth by LLM chatbot service providers?

\item\textbf{RQ2 (Motivation)} How effective are the existing jailbreak prompts against the commercial LLM chatbots?
\end{itemize}

To address \textbf{RQ1}, we prudently assemble a collection of LLM chatbot service providers, recognized for their comprehensive and well-articulated usage policies. We meticulously examine these policies and extract the salient points.
With regards to \textbf{RQ2}, we gather a collection of jailbreak prompts, pulling from both online sources and academic research. These jailbreak prompts are then employed to probe the responses of the targted LLM chatbots. The subsequent analysis of these responses leads to several fascinating observations. In particular, we discover that modern LLM  chatbot services including Bing Chat and Bard implement additional content filtering mechanisms beyond the generative model to enforce the usage policy. Below we detail our empirical study.


\subsection{Usage Policy (RQ1)}\label{sec:study:policy}
Our study encompasses a distinct set of LLM chatbot service providers that satisfy specific criteria. Primarily, we ensure that every provider examined has a comprehensive usage policy that clearly delineates the actions or practices that would be considered violations.
Furthermore, the provider must offer services that are readily available to the public, without restrictions to trial or beta testing periods.
Lastly, the provider must explicitly state the utilization of their proprietary model, as opposed to merely customizing existing pre-trained models with fine-tuning or prompt engineering.
By adhering to these prerequisites, we identify four key service providers fitting our parameters: OpenAI, Bard, Bing Chat, and Ernie.

We meticulously review the content policies~\cite{openai-policy, bard, bing-usage, ERNIE} provided by the four service providers. Following the previous works~\cite{liu2023jailbreaking, li2023multistep}, we manually examine the usage policies to extract and summarize the prohibited usage scenarios stipulated by each provider. Our initial focus centers on OpenAI services, using the restricted categories identified in prior research as a benchmark. We then extend our review to encompass the usage policies of other chatbot services, aligning each policy item with our previously established categories. In instances where a policy item does not conform to our pre-existing categories, we introduce a new category. Through this methodical approach, we delineate 10 restricted categories, which are detailed in Table~\ref{tab:policy}.


To affirm the actual enforcement of these policies, we adopt the methodology in prior research~\cite{liu2023jailbreaking}. Specifically, the authors of this paper work collaboratively to create question prompts for each of the 10 prohibited scenarios. Five question prompts are produced per scenario, ensuring a diverse representation of perspectives and nuances within each prohibited scenario. We feed these questions to the services and validate if they are answered without the usage policy enforcement. The sample questions for each category is presented in the Appendix~\ref{appendix:questions}, while the complete list of the questions is available at our website: \url{https://sites.google.com/view/ndss-masterkey}.



Table~\ref{tab:policy} presents the content policies specified and actually enforced by each service provider. The comparisons across the four providers give some interesting findings. First, all four services uniformly restrict content generation in four prohibited scenarios: illegal usage against law, generation of harmful or abusive contents, violation of rights and privacy, and generation of adult contents. 
This highlights a shared commitment to maintain safe, respectful, and legal usage of LLM services. 
Second, there are mis-allignments of policy specification and actual enforcement. For example, while OpenAI has explicit restrictions on  political campaigning and lobbying, our practice shows that no restrictions are actually implemented on the generated contents. Only Ernie has a policy explicitly forbidding any harm to national security and unity.
%, which likely reflects specific regulatory and cultural contexts in its main market of operations.
In general, these variations likely reflect the different intended uses, regulatory environments, and community norms each service is designed to serve. It underscores the importance of understanding the specific content policies of each chatbot service to ensure compliance and responsible use. 
In the rest of this paper, we primarily focus on four key categories prohibited by all the LLM services. We use \textbf{Illegal}, \textbf{Harmful}, \textbf{Priavcy} and \textbf{Adult} to refer to the four categories for simplicity. %\lyk{only highlight these terms in the table}


\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 1:} There are four common prohibited scenarios restricted by all the mainstream LLM chatbot service providers: illegal usage against law, generation of harmful or abusive contents, violation of rights and privacy, and generation of adult contents.
\end{tcolorbox}

\subsection{Jailbreak Effectiveness (RQ2)}\label{sec:study:effectiveness}
We delve deeper to evaluate the effectiveness of existing jailbreak prompts across different LLM chatbot services.

\noindent\textbf{Target Selection.}
For our empirical study, we focus on four renowned LLM chatbots: OpenAI \gptthree{} and \gptfour{}, Bing Chat, and Google Bard. These services are selected due to their extensive use and considerable influence in the LLM landscape. We do not include Ernie in this study for a couple of reasons. First, although Ernie exhibits decent performance with English content, it is primarily optimized for Chinese, and there are limited jailbreak prompts available in Chinese. A simple translation of prompts might compromise the subtlety of the jailbreak prompt, making it ineffective. Second, we observe  that repeated unsuccessful jailbreak attempts on Ernie result in account suspension, making it infeasible to conduct extensive trial experiments. 
%Owing to this constraint, we refrained from conducting extensive trial experiments on Ernie.


\noindent\textbf{Prompt Preperation.}
We assemble an expansive collection of prompts from various sources, including the website~\cite{jailbreakchat} and research paper~\cite{liu2023jailbreaking}.
As most existing LLM jailbreak studies target OpenAI's GPT models, some prompts are designed with particular emphasis on GPT services.
To ensure a fair evaluation and comparison across different service providers, we adopt a keyword substitution strategy: we replace GPT-specific terms (e.g., ``ChatGPT'', ``GPT'') in the prompts with the corresponding service-specific terms (e.g., ``Bard'', ``Bing Chat Sydney''). 
Ultimately, we collect 85 prompts for our experiment. The complete detail of these prompts are available at our project website: \url{https://sites.google.com/view/ndss-masterkey}.


\noindent\textbf{Experiment Setting.} 
Our empirical study aims to meticulously gauge the effectiveness of jailbreak prompts in bypassing the selected LLM models. To reduce random factors and ensure an exhaustive evaluation, we run each question with every jailbreak prompt for 10 rounds, accumulating to a total of 68,000 queries (5 questions  $\times$ 4 prohibited scenarios $\times$ 85 jailbreak prompts  $\times$ 10 rounds $\times$ 4 models). 
Following the acquisition of results, we conduct a manual review to evaluate the success of each jailbreak attempt by checking whether the response contravenes the identified prohibited scenario.





\noindent\textbf{Results.} Table~\ref{tab:success_count_for_pattern_service} displays the number and ratio of successful attempts for each prohibited scenario. Intriguingly, existing jailbreak prompts exhibit limited effectiveness when applied to models beyond the GPT family. Specifically, while the jailbreak prompts achieve an average success rate of 21.12\% with \gptthree{}, the same prompts yield significantly lower success rates of 0.4\% and 0.63\%  with Bard and Bing Chat, respectively. Based on our observation, there is no existing jailbreak prompt that can consistantly achieve successful jailbreak over Bard and Bing Chat.


\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 2:} The existing jailbreak prompts seems to be effective towards \chatgpt{} only, while demonstrating limited success with Bing Chat and Bard.
\end{tcolorbox}



\begin{table}[t]
\caption{ Number and ratio of successful jailbreaking attempts for different models and scenarios. }
\label{tab:success_count_for_pattern_service}
\centering
\resizebox{\columnwidth}{!}{
%\fontsize{5.5}{10}\selectfont
\begin{tabular}{l||llll||l}
\toprule
\textbf{Pattern} & \textbf{Adult} & \textbf{Harmful} & \textbf{Privacy} & \textbf{Illegal} & \textbf{Average (\%)} \\
\midrule
GPT-3.5   & 400 (23.53\%)             & 243 (14.29\%)               & 423 (24.88\%)               & 370 (21.76\%)           & 359 (21.12\%)                     \\
GPT-4     & 130 (7.65\%)              & 75 (4.41\%)                 & 165 (9.71\%)                & 115 (6.76\%)            & 121.25 (7.13\%)                      \\
Bard      & 2 (0.12\%)                & 5 (0.29\%)                  & 11 (0.65\%)                 & 9 (0.53\%)              & 6.75 (0.40\%)                      \\
Bing Chat & 7 (0.41\%)                & 8 (0.47\%)                  & 13 (0.76\%)                 & 15 (0.88\%)             & 10.75 (0.63\%)        \\
\midrule
Average   & 134.75 (7.93\%)                  & 82.75 (4.87\%)                      & 153 (9.00\%)                      & 127.25 (7.49\%)                  & 124.44 (7.32\%)           \\
\bottomrule
\end{tabular}
}
\end{table}


We further examine the answers to the jailbreak trials, and notice a significant discrepancy in the feedback provided by different LLMs regarding policy violations upon a failed jailbreak. Explicitly, both \gptthree{} and \gptfour{} indicate the precise policies infringed in the response. 
Conversely, other services provide broad, undetailed responses, merely stating their incapability to assist with the request without shedding light on the specific policy infractions. We continue the conversation with the models, questioning the specific violations of the policy. In this case, \gptthree{} and \gptfour{} further ellaborates the policy violated, and provide guidance to users. In contrast, Bing Chat and Bard do not provide any feedback as if the user has never asked a violation question. 


\begin{tcolorbox}[colback=gray!25!white, size=title,breakable,boxsep=1mm,colframe=white,before={\vskip1mm}, after={\vskip0mm}]
\textbf{Finding 3:} OpenAI models including \gptthree{} and \gptfour{}, return the exact policies violated in their responses. This level of transparency is lacking in other services, like Bard and Bing Chat.
\end{tcolorbox}




%we outline our methodical strategy to judiciously reverse engineer these hidden defense mechanisms, setting the stage for our ultimate goal -— a successful jailbreak -— detailed in the upcoming section.

